Hybrid Transformer and CNN Attention Network for Stereo Image Super-resolution

Multi-stage strategies are frequently employed in image restoration tasks. While transformer-based methods have exhibited high efficiency in single-image super-resolution tasks, they have not yet shown significant advantages over CNN-based methods in stereo super-resolution tasks. This can be attributed to two key factors: first, current single-image super-resolution transformers are unable to leverage the complementary stereo information during the process; second, the performance of transformers is typically reliant on sufficient data, which is absent in common stereo-image super-resolution algorithms. To address these issues, we propose a Hybrid Transformer and CNN Attention Network (HTCAN), which utilizes a transformer-based network for single-image enhancement and a CNN-based network for stereo information fusion. Furthermore, we employ a multi-patch training strategy and larger window sizes to activate more input pixels for super-resolution. We also revisit other advanced techniques, such as data augmentation, data ensemble, and model ensemble to reduce overfitting and data bias. Finally, our approach achieved a score of 23.90dB and emerged as the winner in Track 1 of the NTIRE 2023 Stereo Image Super-Resolution Challenge.

==> latex 2/compare_SOTA.tex <==
\begin{table*}[!t]
\caption{Quantitative results achieved by different methods on the KITTI 2012~\cite{Geiger2012CVPR}, KITTI 2015~\cite{Menze2015ISA}, Middlebury~\cite{scharstein2014high}, and Flickr1024~\cite{wang2019learning} datasets. Here, PSNR/SSIM values achieved on both the left images (i.e., Left) and a pair of stereo images (i.e., (Left + Right) /2) are reported. The best results are in \textbf{bold faces}.}
\label{tab:compare}
% \footnotesize
  \renewcommand{\tabcolsep}{3pt}
  \renewcommand{\arraystretch}{1.0} 
\centering	
\begin{tabular}{lccccccc}
    \toprule
    \multirow{2}{*}{Methods} & \multicolumn{3}{c}{\textit{Left}} & \multicolumn{4}{c}{\textit{(Left+Right)/2}} \\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-8}
    & KITTI2012 & KITTI2015 & Middlebury & KITTI2012 & KITTI2015 & Middlebury & Flickr1024 \\
    \midrule
    VDSR~\cite{kim2016accurate} & 25.54/0.7662 & 24.68/0.7456 & 27.60/0.7933 & 25.60/0.7722 & 25.32/0.7703 & 27.69/0.7941 & 22.46/0.6718 \\
    EDSR~\cite{lim2017enhanced} & 26.26/0.7954 & 25.38/0.7811 & 29.15/0.8383 & 26.35/0.8015 & 26.04/0.8039 & 29.23/0.8397 & 23.46/0.7285 \\
    RDN~\cite{zhang2018residual} & 26.23/0.7952 & 25.37/0.7813 & 29.15/0.8387 & 26.32/0.8014 & 26.04/0.8043 & 29.27/0.8404 & 23.47/0.7295 \\
    RCAN~\cite{zhang2018image} & 26.36/0.7968 & 25.53/0.7836 & 29.20/0.8381 & 26.44/0.8029 & 26.22/0.8068 & 29.30/0.8397 & 23.48/0.7286 \\
    SwinIR~\cite{swinir} & 26.43/0.7996 & 25.60/0.7868 & 29.16/0.8379 & 26.52/0.8058 & 26.29/0.8098 & 29.25/0.8385 & 23.53/0.7322\\
    HAT-L~\cite{hat} & 26.91/0.8115 & 26.09/0.8014 & \textbf{30.53/0.8655} & 27.00/0.8177 & 26.83/0.8238 & \textbf{30.65/0.8672} & 24.21/0.7590\\
    \midrule
    StereoSR~\cite{jeon2018enhancing} & 24.49/0.7502 & 23.67/0.7273 & 27.70/0.8036 & 24.53/0.7555 & 24.21/0.7511 & 27.64/0.8022 & 21.70/0.6460 \\
    PASSRnet~\cite{wang2019learning} & 26.26/0.7919 & 25.41/0.7772 & 28.61/0.8232 & 26.34/0.7981 & 26.08/0.8002 & 28.72/0.8236 & 23.31/0.7195 \\
    SRRes+SAM~\cite{ying2020stereo} & 26.35/0.7957 & 25.55/0.7825 & 28.76/0.8287 & 26.44/0.8018 & 26.22/0.8054 & 28.83/0.8290 & 23.27/0.7233 \\
    IMSSRnet~\cite{lei2020deep} & 26.44/- & 25.59/- & 29.02/- & 26.43/- & 26.20/- & 29.02/- & -/- \\
    iPASSR~\cite{ipassr} & 26.47/0.7993 & 25.61/0.7850 & 29.07/0.8363 & 26.56/0.8053 & 26.32/0.8084 & 29.16/0.8367 & 23.44/0.7287 \\
    SSRDE-FNet~\cite{dai2021feedback} & 26.61/0.8028 & 25.74/0.7884 & 29.29/0.8407 & 26.70/0.8082 & 26.43/0.8118 & 29.38/0.8411 & 23.59/0.7352 \\
    Steformer~\cite{10016671} & 26.61/0.8037 & 25.74/0.7906 & 29.29/0.8424 & 26.70/0.8098 & 26.45/0.8134 & 29.38/0.8425 & 23.58/0.7376 \\
    NAFSSR-L~\cite{nafssr} & 27.04/0.8135 & 26.22/0.8034 & 30.11/0.8601 & 27.12/0.8194 & 26.96/0.8257 & 30.20/0.8605 & 24.17/0.7589 \\
    Ours & \textbf{27.16/0.8189} & \textbf{26.26/0.8083} & 30.25/0.8628 & \textbf{27.25/0.8249} & \textbf{26.99/0.8299} & 30.33/0.8634 & \textbf{24.44/0.7703}\\
    \bottomrule
\end{tabular}
% \vspace{-15pt}
\end{table*}

==> latex 2/results.tex <==
\begin{figure*}[ht]
% \vspace{-20pt}
	\footnotesize
% 	\tiny 
% 	\scriptsize        
	\centering
	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
	\renewcommand{\arraystretch}{0.7} % adjust vertical space
	\begin{tabular}{cccc}
	\includegraphics[width=0.23\linewidth]{2.pdf} &
        \includegraphics[width=0.23\linewidth]{2_l.pdf} &
        \includegraphics[width=0.23\linewidth]{2_1.pdf} &
        \includegraphics[width=0.23\linewidth]{2_2.pdf} \\
        \includegraphics[width=0.23\linewidth]{10.pdf} &
        \includegraphics[width=0.23\linewidth]{10_l.pdf} &
        \includegraphics[width=0.23\linewidth]{10_1.pdf} &
        \includegraphics[width=0.23\linewidth]{10_2.pdf} \\
        \includegraphics[width=0.23\linewidth]{13.pdf} &
        \includegraphics[width=0.23\linewidth]{13_l.pdf} &
        \includegraphics[width=0.23\linewidth]{13_1.pdf} &
        \includegraphics[width=0.23\linewidth]{13_2.pdf} \\
         & (a) Bicubic & (b) Transformer-based SISR & (c) CNN-based stereo enhancement \\
        \end{tabular}
	\caption{\textbf{Visual analyses on the proposed multi-stage strategy.} }
	\label{fig:results}
% 	\vspace{-10pt}
\end{figure*}

==> latex 2/sota.tex <==
\begin{figure*}[h!]
% \vspace{-20pt}
	\footnotesize
% 	\tiny 
% 	\scriptsize        
	\centering
	\renewcommand{\tabcolsep}{1.0pt} % adjust horizontal space
	\renewcommand{\arraystretch}{0.7} % adjust vertical space
	\begin{tabular}{ccccc}
	\multirow{2}{*}[9.5em]{\includegraphics[width=0.2\linewidth,height=0.329\linewidth]{7.pdf}} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{lr_7.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{hat_7c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{stereosr_7c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{ipassr_7c.pdf} \\
        & (a) Bicubic & (b) HAT-L~\cite{hat} & (c) StereoSR~\cite{jeon2018enhancing} & (d) iPASSR~\cite{ipassr} \\
        &\includegraphics[width=0.14\linewidth,height=0.228\linewidth]{sam_7c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{naf_7c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{our_7c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{gt_7c.pdf} \\
        & (e) SRRes+SAM~\cite{ying2020stereo} & (f) NAFSSR-L~\cite{nafssr} & Ours & GT \\
        \multirow{2}{*}[9.5em]{\includegraphics[width=0.2\linewidth,height=0.329\linewidth]{19.pdf}} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{lr_19.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{hat_19c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{stereosr_19c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{ipassr_19c.pdf} \\
        & (a) Bicubic & (b) HAT-L~\cite{hat} & (c) StereoSR~\cite{jeon2018enhancing} & (d) iPASSR~\cite{ipassr} \\
        &\includegraphics[width=0.14\linewidth,height=0.228\linewidth]{sam_19c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{naf_19c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{our_19c.pdf} &
        \includegraphics[width=0.14\linewidth,height=0.228\linewidth]{gt_19c.pdf} \\
        & (e) SRRes+SAM~\cite{ying2020stereo} & (f) NAFSSR-L~\cite{nafssr} & Ours & GT \\
        \end{tabular}
	\caption{{\textbf{Visual comparisons on Flickr1024 dataset~\cite{wang2019learning}.} GT denotes the ground truth.} }
	\label{fig:sota}
% 	\vspace{-10pt}
\end{figure*}
